Coarse-to-Fine Curriculum Learning

When faced with learning challenging new tasks, humans often follow sequences of steps that allow them to incrementally build up the necessary skills for performing these new tasks. However, in machine learning, models are most often trained to solve the target tasks directly.Inspired by human learning, we propose a novel curriculum learning approach which decomposes challenging tasks into sequences of easier intermediate goals that are used to pre-train a model before tackling the target task. We focus on classification tasks, and design the intermediate tasks using an automatically constructed label hierarchy. We train the model at each level of the hierarchy, from coarse labels to fine labels, transferring acquired knowledge across these levels. For instance, the model will first learn to distinguish animals from objects, and then use this acquired knowledge when learning to classify among more fine-grained classes such as cat, dog, car, and truck. Most existing curriculum learning algorithms for supervised learning consist of scheduling the order in which the training examples are presented to the model. In contrast, our approach focuses on the output space of the model. We evaluate our method on several established datasets and show significant performance gains especially on classification problems with many labels. We also evaluate on a new synthetic dataset which allows us to study multiple aspects of our method.

==> experiments-blobs.tex <==
\subsubsection{Gaussian blobs}
\paragraph{Dataset generation.}
The goal of this dataset is to provide a task where the labels have an inherent hierarchy, and the label hierarchy is known. For this reason we first create a label hierarchy, and then generate our samples based on it.
The inputs consist of $64 \times 64$ grey-scale images containing a fixed number $k$ of Gaussian blobs. 
Each image is generated using the following generative process:
\begin{enumerate}
    \item Generate the first blob, by selecting randomly a position on the x-axis (between the 20th-80th percentile of the width), a position along the y-axis (between the 20th-80th percentile of the height), and a standard deviation of the Gaussian along the x-axis and y-axis (randomly chosen from a prespecified range).
    \item Select a direction to move along between left (L) or right (R).
    \item If the selected direction is L, the allowed x-axis positions allowed for the next blob are between 0 and the current blob's x coordinate. If the selected direction is R, the allowed x-axis positions allowed for the next blob are between the current blob's x coordinate and the image width.
    \item Repeat steps 1-3 until we obtain $k$ Gaussians.
    \item Create a label for this image consisting of the generated path, which can be represented as a string of length $k$ whose elements are either ``L" or ``R".
\end{enumerate}

This process is shown in Figure~\ref{fig:blobs-explanation}. The arrows start at the fist generated blob, and follow either a left or right direction.
Figure~\ref{fig:blobs} shows some examples of generated images and their corresponding labels.
We show two randomly chosen examples for each label, to illustrate the variability in the input space for the same label.

\begin{figure}[h!]
  \includegraphics[width=\linewidth]{img/blobs-constrained-demo.pdf}
  \caption{Gaussian blobs.}
  \label{fig:blobs}
\end{figure}


\begin{figure}[h!]
  \includegraphics[width=\linewidth]{img/blobs-constrained-explanation.pdf}
  \caption{Image and label generation process.}
  \label{fig:blobs-explanation}
\end{figure}

\paragraph{Results.}
\begin{figure}[h!]
  \includegraphics[width=\linewidth]{img/Accuracy-Gaussian-blobs.pdf}
  \caption{Results on 2D Gaussian blobs data.}
  \label{fig:blobs-results}
\end{figure}

% \input{tables/table-results-blobs.tex}

==> experiments-polygons-no-color.tex <==
\subsubsection{Geometrical Shapes}

\paragraph{Dataset generation.}
The goal of this dataset is to provide a task with a simple set of features where a natural fine-to-coarse curriculum might arise.
The inputs consist of $64 \times 64$ black-and-white images depicting geometrical figures (see Figure~\ref{fig:shapes}).
The shapes include triangles, rectangles, and other regular polygons with arbitrary number of vertices 
The position of the shape within the image, as well as its size and rotation are chosen arbitrarily from a prespecified range.
Given a dataset containing a fixed number of samples per shape, the task is to classify the specific geometrical figure present in each image.

\begin{figure}[h!]
  \includegraphics[width=\linewidth]{img/polygons.pdf}
  \vspace{-1em}
  \caption{Example of polygons included in the dataset.}
  \label{fig:shapes}
\end{figure}

Using the above data, our goal is to classify polygons based on the number of vertices. In this case our samples only contain convex polygons with a number of vertices in \{3, 4, ..., 8, 9, 10\}.
Beyond 10 vertices, the images cannot capture the vertices at this resolution.
The idea behind this generation process is that polygons similar number of vertices should look more alike and thus should be easier for the model to confuse.
Therefore we expect that the model will cluster together polygons with number of vertices that are close to each other.


\begin{figure}[h!]
  \includegraphics[width=\linewidth]{img/plots-acc-difference-polygons.pdf}
  \vspace{-1em}
  \caption{Results on 8 Polygons data.}
  \label{fig:polygons}
\end{figure}

% \input{tables/table-results-shapes.tex}

\paragraph{Model.} 
We use a Convolutional Neural Network (CNN) with 3 convolution layers and 2 linear layers (details in Appendix ).


\paragraph{Results.}
We first run this experiment using baseline model trained without curriculum. As per our method, the confusion matrix of the baseline model is used to compute a label hierarchy, and we group the labels in clusters given by the label hierarchy. Next, we train the model using the current clustering as class labels, as described in Section~\ref{sec:method}, and pretraining the encoder using the model at the previous hierarchy level. Finally, we report the results obtained by the model trained at the last level of the hierarchy (which are the orginal labels), and compare them with the performance of the baseline model.
We perform this experiment multiple times, while varying the number of samples the model is training on.

The results, shown in % Table~\ref{tab:results-shapes} and in 
Figure~\ref{fig:polygons}, indicate that the curriculum approach outperforms the baseline consistently, except when the baseline model is almost perfect ($96.66\%$ accuracy). The plot in Figure~\ref{fig:polygons} suggests that our curriculum approach has most gain in the middle case, when the baseline is neither too good, nor too bad. Intuitively, this makes sense, because if the baseline is too good, there is little to be gained from pretraining, and alternatively, when the baseline performs too poorly (in our case, around $14.5\%$ accuracy), the pretrained model we initialize with at every level of the hierarchy is itself going to be poor, thus affecting the final results.



==> experiments-shapes.tex <==
% \subsubsection{Geometrical Shapes}
In order to study the properties of our method, we created a synthetic dataset that is easy to analyse, and where a natural coarse-to-fine curriculum might arise.
The properties we investigate are:
(i) how our method performs with varying amounts of training data,
(ii) what the class hierarchy looks like, and
(iii) how the class embedding similarity metric compares to other metrics. 

\subsubsection{Dataset Generation.}
We refer to this dataset as \dataset{Shapes}.
The inputs consist of $64 \times 64$ images depicting one of 10 geometrical shapes (circles, ellipses, and regular polygons with 3-10 vertices) with one of three colors (magenta, cyan, or grey) against a black background (see Figure~\ref{fig:shapes}).
%The position of each shape within an image, its size and its rotation angle are chosen randomly from a pre-specified range, as well as its color.
The generated dataset contains $50,000$ images ($5,000$ per shape), out of which we set $10,000$ aside for testing.
We have made both the dataset and generation code available at {\small \url{http://www.anonymous.com}}.
%{\small \url{https://github.com/otiliastr/coarse-to-fine-curriculum}}.
% The task is to classify the specific shape in each image, and shapes of different color have distinct labels (i.e., the model must learn to distinguish between a grey and magenta triangle).
The task is to classify the specific shape and color combination in each image (i.e., we have 30 classes). % and shapes of different color have distinct labels (i.e., the model must learn to distinguish between a grey and magenta triangle).
% Thus, this classification task involves 30 classes.
The idea behind this dataset is that shapes with similar color and number of vertices look more alike and thus are more likely to confuse the model.
We expect our method to provide a significant performance boost in this setting because it resembles the main motivation behind it.

\subsubsection{Results.}
We performed experiments with the \model{CNN} architecture.
Our results, shown in Figure~\ref{fig:polygons-only-cont}, indicate that our method outperforms the baseline consistently. % except for when the baseline is very poor ($13\%$ accuracy).
% After investigating into what caused this we made two observations:
% (i) when the baseline performs too poorly, the confusion matrix used to obtain our class hierarchy is also very poor, resulting in the curriculum method not offering a significant performance boost, and
% (ii) there is a point at which the amount of labeled data is too little to actually allow any model to learn something meaningful; at that point we do not expect our curriculum approach to offer any significant boost in performance over the baseline method.
% This expected, because if the baseline performs too poorly, then the pre-trained model we initialize with at every level of the hierarchy is itself going to be poor, thus affecting the final results.
Furthermore, we observe that the curriculum method provides the biggest boost over the baseline in the middle regime, when there are not enough samples for the baseline to reach high accuracy, but there is enough to make it a sufficiently good learner that our curriculum learning algorithm can improve upon.
These results also agree with previous results showing that pre-training is most beneficial in problems where labeled data is scarce.
% Comparing the two versions of the curriculum, the continuous approach seems to consistently outperform the staged one.
% This result confirms our intuition for proposing the continuous approach, which was that it is useful to reuse the predictor parameters, $\theta^\texttt{pred}$, from the previous hierarchy levels.
To further understand where the gains are coming from, we also inspected the generated label hierarchy.
% The most common hierarchy generated during the experiments is the following:
% \uline{Level 1:} The shapes are grouped by color into 3 clusters.
% \uline{Level 2:} There are 6 clusters:
% \texttt{\footnotesize [cyan circle,cyan ellipse]},
% \texttt{\footnotesize [cyan polygon\textsuperscript{3},cyan polygon\textsuperscript{4},...,cyan polygon\textsuperscript{10}]},
% \texttt{\footnotesize [gray circle,gray ellipse]},
% \texttt{\footnotesize [gray polygon\textsuperscript{3},gray polygon\textsuperscript{4},...,gray polygon\textsuperscript{10}]},
% \texttt{\footnotesize [magenta circle,magenta ellipse]},
% \texttt{\footnotesize [magenta polygon\textsuperscript{3},magenta polygon\textsuperscript{4},...,magenta polygon\textsuperscript{10}]}, 
% where \texttt{\footnotesize polygon\textsuperscript{$k$}} denotes a polygon with $k$ vertices.
% \underline{Level 3:} Each shape has its own class.
The most common hierarchy generated during the experiments separates all shapes by color on the first level, and by shape similarity on the second level (i.e., circles and ellipses are grouped together, and all polygons are grouped together).
This is intuitive and compatible with what a human could have constructed.

% CIFAR PLOT
% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{img/plots-acc-difference.pdf}
%     \caption{Accuracy difference between the baseline model and a model trained with a coarse-to-fine curriculum.}
%     \label{fig:acc-difference}
% \end{figure*}

\subsubsection{Similarity Metric Evaluation.}
A natural question to ask is whether using the class embedding similarity as a similarity metric between classes is better than alternative approaches.
For example, what if we force classes that are similar to be separated into different clusters early on?
% Could this help the model focus on them earlier and learn to handle them better?
To answer this question, we also tested our approach by replacing the class embedding distance metric with:
(i) the class confusion matrix (\dataset{Confusion}),
(ii) a similarity matrix defined as 1 minus the confusion matrix (\dataset{ConfusionSim}),
(iii) the class embedding distance used in the rest of our experiments (\dataset{EmbeddingDist}),
(iv) the class embedding similarity (\dataset{EmbeddingSim}), and
(v) a completely random grouping of the classes (\dataset{Random}).
The results---obtained using the continuous curriculum---are presented in Table~\ref{tab:results-shapes-random}.
% Another natural concern is whether the curriculum itself indeed matters, or the model can simply benefit from any clustering of the labels. This could be because assigning coarse group labels to samples still requires learning feature representations that distinguish these groups (e.g., edges, corners), no matter what the grouping is. We also test this hypothesis by replacing the confusion matrix with a random symmetrical matrix, whose elements are drawn from a Gaussian distribution with mean 0 and standard deviation 1. The results are indicated by ``random" in Table~\ref{tab:results-shapes-random}.
We observe that \dataset{Random} hurts performance, and the same is true for the metrics that group dissimilar classes early on.
On the other hand, \dataset{EmbeddingDist} and \dataset{Confusion} both result in large accuracy boosts, with the former resulting in the largest gain.
This is intuitive and also suggests that using arbitrary hierarchies along with our curriculum is not sufficient; {\em the actual choice of class hierarchy matters}.


==> experiments-vectors.tex <==
\subsubsection{Continuous vectors}
\paragraph{Dataset generation.} TODO
\paragraph{Results.}
\begin{figure*}[h!]
  \includegraphics[width=\linewidth]{img/accuracy-Gaussian-vector-inputs.pdf}
  \caption{Results on continuous vectors data.}
  \label{fig:results-vectors}
\end{figure*}


==> tables/results-continuous-real-confusion.tex <==

% \begin{table*}[t!]
%     \caption{
% 	    Results on real classification datasets.
% 	    We show the accuracy mean and standard error for the baseline and the model trained with curriculum, over 5 runs initialized with random seeds, as well as their difference, computed per run and then averaged.}
% 	\label{tab:results-single-label}
% 	\vspace{1ex}
%     \centering
% 	\scriptsize
% 	\lato
% 	\def\arraystretch{1.2}
% 	\setlength{\tabcolsep}{10pt}
% 	\begin{tabularx}{\textwidth}{|lrr||Y|Y|Y|}
% 	    \hhline{|---||---|}
% 	    \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\#Classes}} & \multirow{2}{*}{\textbf{\#Samples}} & \multicolumn{3}{c|}{\textbf{Accuracy}} \\
% 	    \hhline{|~~~||---|}
% 	    & & & \textbf{Baseline} & \textbf{Curriculum} & \textbf{Difference} \\
% 	   \hhline{:===::===:}
% 	    CIFAR-10 & 10 & 50,000 & 70.82 $\pm$ 0.14 & \textbf{71.31 $\pm$ 0.08} & \diff{0.50}{0.21} \\
%         CIFAR-10 & 10 & 20,000 & 64.61 $\pm$ 0.40 & \textbf{65.23 $\pm$ 0.14} & \diff{0.62}{0.51} \\
%         CIFAR-10 & 10 & 10,000 & 59.25 $\pm$ 0.34 & \textbf{59.86 $\pm$ 0.35} & \diff{0.61}{0.54} \\
%         CIFAR-10 & 10 &  5,000 & 53.35 $\pm$ 0.27 & \textbf{53.53 $\pm$ 0.29} & \diff{0.18}{0.43} \\
%         \hhline{:===::===:}
%         CIFAR-100 Coarse & 20 & 50,000 & 49.40 $\pm$ 0.37 & \textbf{50.81 $\pm$ 0.36} & \diff{1.41}{0.64} \\
%         CIFAR-100 Coarse & 20 & 20,000 & 41.97 $\pm$ 0.17 & \textbf{43.27 $\pm$ 0.27} & \diff{1.31}{0.17} \\
%         CIFAR-100 Coarse & 20 & 10,000 & 36.79 $\pm$ 0.21 & \textbf{38.34 $\pm$ 0.17} & \diff{1.56}{0.34} \\
%         CIFAR-100 Coarse & 20 &  5,000 & 31.80 $\pm$ 0.34 & \textbf{33.18 $\pm$ 0.47} & \diff{1.39}{0.52} \\
%         \hhline{:===::===:}
%         CIFAR-100 & 100 & 50,000 & 35.97 $\pm$ 0.32 & \textbf{39.58 $\pm$ 0.35} & \diff{3.62}{0.26} \\
%         CIFAR-100 & 100 & 20,000 & 27.71 $\pm$ 0.36 & \textbf{30.21 $\pm$ 0.44} & \diff{2.51}{0.16} \\
%         CIFAR-100 & 100 & 10,000 & 22.02 $\pm$ 0.27 & \textbf{24.19 $\pm$ 0.22} & \diff{2.17}{0.35} \\
%         CIFAR-100 & 100 &  5,000 & 17.32 $\pm$ 0.16 & \textbf{18.78 $\pm$ 0.49} & \diff{1.45}{0.38} \\
% 	   % SVHN     &  10  & 73,257 & \textbf{89.79 $\pm$ 0.12}   & 89.63 $\pm$ 0.10 & \diff{-0.17}{0.04} \\
%     %     SVHN     &  10  & 20,000 & \textbf{86.06 $\pm$ 0.28} & 85.88 $\pm$ 0.39 & \diff{-0.17}{0.63} \\
%     %     SVHN     &  10  & 10,000 & \textbf{84.03 $\pm$ 0.32} & 83.74 $\pm$ 0.39 & \diff{-0.19}{0.09} \\
%     %     SVHN     &  10  &  5,000 & \textbf{81.66 $\pm$ 0.13} & 81.51 $\pm$ 0.54 & \diff{-0.15}{0.42} \\
%     %     SVHN     &  10  &  1,000 & 69.21 $\pm$ 0.27 & \textbf{72.46 $\pm$ 0.31} & \uline{\diff{3.25}{0.44}} \\
%     %     SVHN     &  10  &    500 & 60.06 $\pm$ 0.82 & \textbf{64.71 $\pm$ 0.76} & 
%     %     \uline{\diff{4.65}{0.25}} \\
%     %     SVHN     &  10  &    100 & 20.27 $\pm$ 0.90 & \textbf{20.79 $\pm$ 1.30 } & \diff{2.07}{0.84} \\
%         \hhline{:===::===:}
%         Tiny-ImageNet & 200 & 100,000 &           21.93 $\pm$ 0.20 & \textbf{          23.98 $\pm$ 0.20} & \diff{2.05}{0.2} \\
%         % Tiny-ImageNet & 200 &  50,000 &           15.26 $\pm$ 0.25 & \textbf{          22.20 $\pm$ 0.42} & \diff{6.94}{0.18} \\
%         Tiny-ImageNet & 200 &  20,000 &           10.38 $\pm$ 0.14 & \textbf{          11.94 $\pm$ 0.23} & \diff{1.56}{0.24} \\
%         Tiny-ImageNet & 200 &  10,000 & \phantom{0}7.20 $\pm$ 0.11 & \textbf{\phantom{0}7.91 $\pm$ 0.08} & \diff{0.71}{0.16} \\
%         Tiny-ImageNet & 200 &   5,000 & \phantom{0}4.80 $\pm$ 0.25 & \textbf{\phantom{0}5.51 $\pm$ 0.21} & \diff{0.71}{0.20} \\
%     \hhline{|---||---|}
% 	\end{tabularx}
% 	\vspace{-3ex}
% \end{table*}


\begin{table*}[t!]
\caption{
    Results on real classification datasets.
    We show the accuracy mean and standard error for the baseline and the model trained with curriculum, over 5 runs initialized with random seeds, as well as their difference, computed per run and then averaged.}
\label{tab:results-single-label}
\vspace{1ex}
\centering
\tiny
\lato
\def\arraystretch{1.2}
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\textwidth}{|p{1.3cm}p{0.4cm}r||Y||Y|Y||Y|Y||Y|Y|}
    \hhline{|---||-||--||--||--|}
    \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\#Class}} & \multirow{2}{*}{\textbf{\#Samples}} & \textbf{Accuracy} & \multicolumn{2}{c||}{\textbf{Accuracy Staged}} & \multicolumn{2}{c||}{\textbf{Accuracy Continuous}} & \multicolumn{2}{c|}{\textbf{Accuracy Data Params}} \\
    \hhline{|~~~||~||--||--||--|}
    & & & \textbf{Baseline} & \textbf{Curriculum} & \textbf{Difference} & \textbf{Curriculum} & \textbf{Difference} & \textbf{Curriculum} & \textbf{Difference} \\
   \hhline{:===::=::==::==::==:}
    CIFAR-10 & 10 &    50,000 & 70.82 $\pm$ 0.14 & 71.81 $\pm$ 0.07 &  \diff{0.73}{0.25} & \textbf{71.31 $\pm$ 0.08} & \diff{0.50}{0.21} & & \\
    CIFAR-10 & 10 &    20,000 & 64.61 $\pm$ 0.40 & 64.92 $\pm$ 0.34 & \diff{-0.07}{0.41} & \textbf{65.23 $\pm$ 0.14} & \diff{0.62}{0.51} & &\\
    CIFAR-10 & 10 &    10,000 & 59.25 $\pm$ 0.34 & 61.42 $\pm$ 0.27 &  \diff{0.48}{0.19} & \textbf{59.86 $\pm$ 0.35} & \diff{0.61}{0.54} & &\\
    CIFAR-10 & 10 &     5,000 & 53.35 $\pm$ 0.27 & 56.84 $\pm$ 0.42 &  \diff{0.95}{0.36} & \textbf{53.53 $\pm$ 0.29} & \diff{0.18}{0.43} & &\\
    \hhline{:===::=::==::==::==:}
    CIFAR-100 C & 20 & 50,000 & 49.40 $\pm$ 0.37 & 50.38 $\pm$ 0.13 &  \diff{0.69}{0.35} & \textbf{50.81 $\pm$ 0.36} & \diff{1.41}{0.64} & &\\
    CIFAR-100 C & 20 & 20,000 & 41.97 $\pm$ 0.17 & 42.04 $\pm$ 0.15 & \diff{-0.23}{0.31} & \textbf{43.27 $\pm$ 0.27} & \diff{1.31}{0.17} & &\\
    CIFAR-100 C & 20 & 10,000 & 36.79 $\pm$ 0.21 & 39.12 $\pm$ 0.28 &  \diff{1.15}{0.38} & \textbf{38.34 $\pm$ 0.17} & \diff{1.56}{0.34} & &\\
    CIFAR-100 C & 20 &  5,000 & 31.80 $\pm$ 0.34 & 35.12 $\pm$ 0.25 &  \diff{1.60}{0.50} & \textbf{33.18 $\pm$ 0.47} & \diff{1.39}{0.52} & &\\
    \hhline{:===::=::==::==::==:}
    CIFAR-100 & 100 & 50,000  & 36.07 $\pm$ 0.33 & 40.93 $\pm$ 0.25 &  \diff{4.38}{0.25} & \textbf{39.19 $\pm$ 0.42} & \diff{3.12}{0.18} & &\\
    CIFAR-100 & 100 & 20,000  & 27.64 $\pm$ 0.34 & 32.82 $\pm$ 0.63 &  \diff{3.14}{0.55} & \textbf{30.01 $\pm$ 0.31} & \diff{2.36}{0.27} & &\\
    CIFAR-100 & 100 & 10,000  & 22.30 $\pm$ 0.33 & 27.66 $\pm$ 0.26 &  \diff{2.99}{0.73} & \textbf{24.05 $\pm$ 0.34} & \diff{1.75}{0.48} & &\\
    CIFAR-100 & 100 &  5,000  & 17.12 $\pm$ 0.34 & 22.50 $\pm$ 0.48 &  \diff{4.24}{0.41} & \textbf{19.08 $\pm$ 0.33} & \diff{1.96}{0.28} & &\\
    % \hhline{:===::=::==::==:}
    % Tiny-ImageNet & 200 & 100,000 &  18.95 $\pm$ 0.87 & \textbf{          25.43 $\pm$ 0.20} & \diff{6.48}{0.67}&          21.93 $\pm$ 0.20 & \textbf{          23.98 $\pm$ 0.20} & \diff{2.05}{0.2} \\
    % Tiny-ImageNet & 200 &  50,000 &           15.26 $\pm$ 0.25 & \textbf{          22.20 $\pm$ 0.42} & \diff{6.94}{0.18} & 16.09 $\pm$ 0.17 & 18.54 $\pm$ 0.19 & \diff{2.45}{0.29} \\
    % Tiny-ImageNet & 200 &  20,000 &          12.14 $\pm$ 0.15 & \textbf{          15.65 $\pm$ 0.05} & \diff{3.51}{0.17} &          10.38 $\pm$ 0.14 & \textbf{          11.94 $\pm$ 0.23} & \diff{1.56}{0.24} \\
    % Tiny-ImageNet & 200 &  10,000 & {\leavevmode\hphantom{0}}8.51 $\pm$ 0.06 & \textbf{          10.85 $\pm$ 0.29} & \diff{2.35}{0.35} &\phantom{0}7.20 $\pm$ 0.11 & \textbf{\phantom{0}7.91 $\pm$ 0.08} & \diff{0.71}{0.16} \\
    % Tiny-ImageNet & 200 &   5,000 &  {\leavevmode\hphantom{0}}6.34 $\pm$ 0.11 & {\leavevmode\hphantom{0}}\textbf{7.94 $\pm$ 0.15} & \diff{1.60}{0.13}  &\phantom{0}4.80 $\pm$ 0.25 & \textbf{\phantom{0}5.51 $\pm$ 0.21} & \diff{0.71}{0.20} \\
\hhline{|---||-||--||--||--|}
\end{tabularx}
\vspace{-3ex}
\end{table*}

==> tables/results-continuous-real.tex <==
% These results use the class embedding difference.

\begin{table*}[t!]
% \vspace{-1.5em}
\centering
\scriptsize
\lato
% \def\arraystretch{1.0}
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\textwidth}{|c|lcr||Y||Y|Y|Y|Y|Y||Y|}
    \hhline{|-|---||-||------|}
    \multirow{2.5}{*}{\textbf{Model}} & \multirow{2.5}{*}{\textbf{Dataset}} & \multirow{2.5}{*}{\textbf{\#Class}} & \multirow{2.5}{*}{\textbf{\#Samples}} & \textbf{Accuracy (\%)} & \multicolumn{6}{c|}{\textbf{Accuracy Gain (\%)}} \\
    \hhline{|~|~~~|:=::=====:t:=:}
    & &    &        & \textbf{Baseline}& \textbf{SPL}      & \textbf{DP-L} & \textbf{DP-LI} &  \textbf{TreeLoss} &  \textbf{NBDT} & \textbf{Coarse-to-Fine} \\
    \hhline{:=:===::=::=:=:=:=:=::=:}
    \multirow{16}{*}{\STAB{\rotatebox[origin=c]{90}{\texttt{CNN}}}} 
    % \multirow{16}{*}{\texttt{CNN}} 
    &CIFAR-10 & 10 & 50,000 & 70.92 $\pm$ 0.37 & \diff{-0.04}{0.19} &  \diff{0.26}{0.20} & \diff{0.53}{0.30} & \diff{0.12}{0.25} &  & \diff{0.69}{0.32} \\
    &CIFAR-10 & 10 & 20,000 & 64.66 $\pm$ 0.53 & \diff{0.14}{0.17}  & \diff{-0.05}{0.46} & \diff{0.07}{0.10} &                   &  & \diff{1.28}{0.60} \\
    &CIFAR-10 & 10 & 10,000 & 59.52 $\pm$ 0.35 & \diff{-0.26}{0.25} &  \diff{0.21}{0.55} & \diff{0.84}{0.41} &                   &  & \diff{1.24}{0.46} \\
    &CIFAR-10 & 10 & {\leavevmode\hphantom{0}}5,000 & 53.64 $\pm$ 0.19 &  \diff{0.89}{1.11} & \diff{-0.54}{0.52} & \diff{-0.48}{0.20} & &  & \diff{1.57}{0.39} \\
    \hhline{|~|---||-||-|-|-|-|-||-|}
    &CIFAR-100 Coarse & 20 & 50,000 & 49.63 $\pm$ 0.35 & \diff{-0.27}{0.09} & \diff{-0.65}{0.34} & \diff{-0.75}{0.47} & \diff{-0.08}{0.24} &  & \diff{1.22}{0.38} \\
    &CIFAR-100 Coarse & 20 & 20,000 & 42.04 $\pm$ 0.29 &  \diff{0.12}{0.36} & \diff{-1.14}{0.06} & \diff{-0.66}{0.10} &                    &  & \diff{1.84}{0.51} \\
    &CIFAR-100 Coarse & 20 & 10,000 & 36.61 $\pm$ 0.19 &  \diff{0.17}{0.16} & \diff{-0.83}{0.23} & \diff{-0.98}{0.29} &                    &  & \diff{1.77}{0.56} \\
    &CIFAR-100 Coarse & 20 & {\leavevmode\hphantom{0}}5,000 & 31.80 $\pm$ 0.28 & \diff{0.26}{0.31} & \diff{-0.91}{0.49} & \diff{-0.51}{0.38} & &  & \diff{1.38}{0.22} \\
    \hhline{|~|---||-||-|-|-|-||-|}
    &CIFAR-100 & 100 & 50,000 & 35.87 $\pm$ 0.23 &  \diff{0.94}{0.61} &  \diff{0.14}{0.25} &  \diff{0.26}{0.31} & \diff{0.69}{0.15} &  & \diff{3.31}{0.59} \\
    &CIFAR-100 & 100 & 20,000 & 27.83 $\pm$ 0.34 &  \diff{0.11}{0.20} & \diff{-0.19}{0.10} & \diff{-0.28}{0.24} & \diff{0.57}{0.48} &  & \diff{2.27}{0.37} \\
    &CIFAR-100 & 100 & 10,000 & 21.96 $\pm$ 0.49 & \diff{-0.32}{0.38} & \diff{-0.12}{0.28} & \diff{-0.06}{0.32} & \diff{0.15}{0.54} &  & \diff{2.67}{0.68} \\
    &CIFAR-100 & 100 & {\leavevmode\hphantom{0}}5,000 & 17.20 $\pm$ 0.20 & \diff{-0.13}{0.23} &\diff{0.25}{0.25} & \diff{0.02}{0.11} & \diff{0.53}{0.19} &  & \diff{1.92}{0.24} \\
    \hhline{|~|---||-||-|-|-|-|-||-|}
    &Tiny-ImageNet & 200 &                         100,000 & 21.94 $\pm$ 0.19 & \diff{-0.97}{0.97} & \diff{-0.05}{0.14} & \diff{-0.08}{0.15} & \diff{0.33}{0.33} &  &  \diff{2.73}{0.49} \\
    &Tiny-ImageNet & 200 & {\leavevmode\hphantom{0}}50,000 & 16.33 $\pm$ 0.32 &  \diff{0.27}{0.30} & \diff{-0.28}{0.12} & \diff{-0.38}{0.15} &                   &   & \diff{3.06}{0.33} \\
    &Tiny-ImageNet & 200 & {\leavevmode\hphantom{0}}20,000 & 10.16 $\pm$ 0.22 &  \diff{0.06}{0.26} &  \diff{0.19}{0.14} &  \diff{0.17}{0.17} &                   &  & \diff{2.02}{0.34} \\
    &Tiny-ImageNet & 200 & {\leavevmode\hphantom{0}}10,000 & {\leavevmode\hphantom{0}}7.38 $\pm$ 0.11 & \diff{-0.22}{0.19} &\diff{0.12}{0.04} & \diff{-0.04}{0.07} & &  &  \diff{1.14}{0.19} \\
    \hhline{:=:===::=::=:=:=:=:=::=:}
    \multirow{8}{*}{\STAB{\rotatebox[origin=c]{90}{\texttt{Resnet18}}}} 
    % \multirow{8}{*}{\texttt{Resnet18}}
    & CIFAR-100    & 200  & 50,000    & 74.84 $\pm$ 0.49 & &                &                & & \diff{-1}{} & \diff{0.92}{0.22} \\
    & CIFAR-100    & 200  & 20,000    & 61.24 $\pm$ 0.21 & &                &                & &  & \diff{2.73}{0.41} \\
    & CIFAR-100    & 200  & 10,000    & 46.01 $\pm$ 0.91 & &                &                & &  & \diff{4.61}{0.40} \\
    % & CIFAR-100    & 200  &  5,000    & & &                &                & & \diff{2.32}{0.97} \\
    \hhline{|~|---||-||-|-|-|-|-||-|}
    % &ImageNet    & 1000 & 1,281,167 & 70.30 $\pm$ 0.10 & --- &  \diff{0.50}{0.20} &  \diff{0.70}{0.20} & &\\ 
    &Tiny-ImageNet & 200  & 100,000   & 43.28 $\pm$ 0.12 & --- & \diff{-0.37}{0.23} & \diff{-0.28}{0.30} & \diff{0.84}{0.35} &  & \diff{2.60}{0.23} \\
    &Tiny-ImageNet & 200  & 50,000    & 35.91 $\pm$ 0.08 & --- & \diff{-0.10}{0.08} & \diff{-0.05}{0.11} & &  & \diff{1.42}{0.36} \\
    &Tiny-ImageNet & 200  & 20,000    & 25.35 $\pm$ 0.31 & --- & \diff{-0.70}{0.20} & \diff{-0.73}{0.17} & &  & \diff{1.27}{0.45}  \\
    &Tiny-ImageNet & 200  & 10,000    & 16.93 $\pm$ 0.14 & --- & ---                & ---                & &  & \diff{2.10}{0.41}  \\
    \hhline{:=:===::=::=:=:=:=:=::=:}
    \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{\texttt{Resnet50}}}} 
    & CIFAR-100    & 200  & 50,000    & & &                &                & &  & \diff{0.50}{0.11} \\
    & CIFAR-100    & 200  & 10,000    & & &                &                & &  & \diff{0.68}{0.19} \\
    & CIFAR-100    & 200  &  5,000    & & &                &                & &  & \diff{2.09}{1.61} \\
    % \multirow{8}{*}{\texttt{Resnet50}}
    \hhline{:=:===::=::=:=:=:=:=::=:}
    % \multirow{4}{*}{\texttt{WideResnet-28-10}} 
    \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{\texttt{WRN-28-10}}}} 
    &CIFAR-100 & 100 & 50,000 & 80.10 $\pm$ 0.20 & --- & --- & \diff{0.7}{0.10} & \diff{-0.21}{} &  & \diff{0.55}{0.13} \\
    &CIFAR-100 & 100 & 10,000 & 58.72 $\pm$ 0.38 & --- & --- &  ---             & &  & \diff{1.29}{0.35} \\
    &CIFAR-100 & 100 &  5,000 & 43.77 $\pm$ 0.98 & --- & --- &  ---             & &  & \diff{2.49}{0.90} \\
    &CIFAR-100 & 100 &  1,000 & 14.87 $\pm$ 0.14 & --- & --- &  ---             & &  & \diff{0.54}{0.56} \\
    \hhline{|-|---||-||-|-|-|-|-||-|}
\end{tabularx}
\caption{
    Results on real datasets, showing the accuracy mean and standard error for the baseline model, computed over 5 runs, as well as the accuracy gain achieved by the various curriculum approaches, computed per run and then averaged.
    \dataset{\small DP-L} and \dataset{\small DP-LI} refer to the curriculum proposed by \citet{saxena2019data}, over labels or over labels and instances, respectively.
    \dataset{\small SPL} refers to self-paced learning \citep{kumar2010self}.
    \dataset{\small Coarse-to-Fine} refers to our algorithm.
    For computational reasons, for the larger models we did not evaluate all competitors (missing results are marked as ``--'').
    For the numbers we do report, we tried several hyperparameter configurations starting with the ones reported in the original publications (\dataset{\small DP-L} and \dataset{\small DP-LI} have 3 and 6 curriculum-specific hyperparameters, respectively).
    %The \dataset{\small DP-L} and \dataset{\small DP-LI} results for \model{WideResnet} are borrowed from the original publication.
}
\label{tab:results-single-label}
% \vspace{-4.0ex}
\end{table*}


==> tables/results-real-multilabel.tex <==
\begin{table*}[t!]
 \centering
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
      \multirow{2}{*}{\textbf{Dataset}} &
      \multicolumn{2}{c|}{\textbf{MicroF1}} & \multicolumn{2}{c|}{\textbf{MacroF1}}  & \multicolumn{2}{c|}{\textbf{Hamming Loss}} &
      \multicolumn{2}{c|}{\textbf{Prec@1}} &  
      \multicolumn{2}{c|}{\textbf{Prec@5}} & 
      \multicolumn{2}{c}{\textbf{Prec@10}} \\ 
      
      &  \textbf{baseline} & \textbf{curric}
      &  \textbf{baseline} & \textbf{curric}
      &  \textbf{baseline} & \textbf{curric}
      &  \textbf{baseline} & \textbf{curric}
      &  \textbf{baseline} & \textbf{curric}
      &  \textbf{baseline} & \textbf{curric}\\
      \hline
      
      Bibtex  & 59.68 & \textbf{69.5} 
              & 50.22 & \textbf{64.52} 
              & 0.0105 & \textbf{0.0086}
              & 73.44 & \textbf{75.71}
              & 32.48 & \textbf{34.33} 
              & 18.44 & \textbf{19.22}  \\
      Mediamill & 57.68  & \textbf{60.86}
                & 8.01   & \textbf{16.42}
                & 0.0296 & \textbf{0.0280} 
                & 84.59  & \textbf{86.32}
                & 53.26  & \textbf{55.19}
                & 34.25  & \textbf{35.19} \\
      Delicious & 37.97 & \textbf{39.64}
                & \textbf{15.03} & 14.04
                & 0.0168 & \textbf{0.0166}
                & 75.67 & \textbf{76.54}
                & 66.07 & \textbf{67.03}
                & 56.4 & \textbf{56.7}
    \end{tabular}
    \end{adjustbox}
  \caption{Results on multilabel datasets.}
   \label{tab:results-multilabel}
\end{table*}


==> tables/results-real-single-label.tex <==
% \begin{table}[ht]
%         \begin{center}
%             \begin{tabular}{*{10}{R}}
%               0.73 & 1.00 & 1.00 & 1.00 & 0.99 & 0.98 & 0.96 & 0.90 & 0.82 & 0.37 \\
%               1.00 & 1.00 & 0.99 & 0.98 & 0.95 & 0.90 & 0.82 & 0.61 & 0.37 & 0.01 \\
%               1.00 & 0.99 & 0.98 & 0.96 & 0.90 & 0.82 & 0.67 & 0.37 & 0.14 & 0.00 \\
%               1.00 & 0.98 & 0.95 & 0.90 & 0.78 & 0.61 & 0.37 & 0.08 & 0.01 & 0.00 \\
%               0.99 & 0.95 & 0.90 & 0.82 & 0.61 & 0.37 & 0.14 & 0.01 & 0.00 & 0.00 \\
%               0.98 & 0.90 & 0.82 & 0.67 & 0.37 & 0.14 & 0.02 & 0.00 & 0.00 & 0.00 \\
%               0.95 & 0.78 & 0.61 & 0.37 & 0.08 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\
%               0.90 & 0.61 & 0.37 & 0.14 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
%               0.82 & 0.37 & 0.14 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
%               0.37 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
%             \end{tabular}
%         \end{center}
%     \end{table}
    
\begin{table*}[t!]
    \caption{
	    Results on real classification datasets.
	    We show the accuracy mean and standard error for the baseline and the model trained with curriculum, over 5 runs initialized with random seeds, as well as their difference, computed per run and then averaged.}
	\label{tab:results-single-label}
	\vspace{1ex}
    \centering
	\scriptsize
	\lato
	\def\arraystretch{1.2}
	\setlength{\tabcolsep}{10pt}
	\begin{tabularx}{\textwidth}{|lrr||Y|Y|Y|}
	    \hhline{|---||---|}
	    \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\#Classes}} & \multirow{2}{*}{\textbf{\#Samples}} & \multicolumn{3}{c|}{\textbf{Accuracy}} \\
	    \hhline{|~~~||---|}
	    & & & \textbf{Baseline} & \textbf{Curriculum} & \textbf{Difference} \\
	    \hhline{:===::===:}
	    SVHN     &  10  & 73,257 & \textbf{89.79 $\pm$ 0.12}   & 89.63 $\pm$ 0.10 & \diff{-0.17}{0.04} \\
        SVHN     &  10  & 20,000 & \textbf{86.06 $\pm$ 0.28} & 85.88 $\pm$ 0.39 & \diff{-0.17}{0.63} \\
        SVHN     &  10  & 10,000 & \textbf{84.03 $\pm$ 0.32} & 83.74 $\pm$ 0.39 & \diff{-0.19}{0.09} \\
        SVHN     &  10  &  5,000 & \textbf{81.66 $\pm$ 0.13} & 81.51 $\pm$ 0.54 & \diff{-0.15}{0.42} \\
        SVHN     &  10  &  1,000 & 69.21 $\pm$ 0.27 & \textbf{72.46 $\pm$ 0.31} & \uline{\diff{3.25}{0.44}} \\
        SVHN     &  10  &    500 & 60.06 $\pm$ 0.82 & \textbf{64.71 $\pm$ 0.76} & 
        \uline{\diff{4.65}{0.25}} \\
        SVHN     &  10  &    100 & 20.27 $\pm$ 0.90 & \textbf{20.79 $\pm$ 1.30 } & \diff{2.07}{0.84} \\
        \hhline{:===::===:}
        % converted to std error
        CIFAR-10 & 10  & 50,000 &          71.08 $\pm$ 0.22 & \textbf{71.81 $\pm$ 0.07} &  \uline{\diff{0.73}{0.25}} \\
        CIFAR-10 & 10  & 20,000 & \textbf{64.99 $\pm$ 0.25} &         64.92 $\pm$ 0.34  & \diff{-0.07}{0.41} \\
        CIFAR-10 & 10  & 10,000 &          60.94 $\pm$ 0.19 & \textbf{61.42 $\pm$ 0.27} & \diff{0.48}{0.19} \\
        CIFAR-10 & 10  &  5,000 &          55.89 $\pm$ 0.37 & \textbf{56.84 $\pm$ 0.42} & \diff{0.95}{0.36} \\
        CIFAR-10 & 10  &  1,000 &          42.52 $\pm$ 0.64 & \textbf{43.78 $\pm$ 0.23} & \diff{1.26}{0.61} \\
        CIFAR-10 & 10  &    500 &          37.75 $\pm$ 0.56 & \textbf{39.23 $\pm$ 0.68} & \diff{1.47}{0.37} \\
        CIFAR-10 & 10  &    100 &          24.81 $\pm$ 0.76 & \textbf{27.69 $\pm$ 0.31} & \diff{2.87}{0.80} \\
        \hhline{:===::===:}
        % converted to std error
        CIFAR-100 Coarse & 20 & 50,000 &         49.55 $\pm$ 0.32  & \textbf{50.38 $\pm$ 0.13} & \diff{0.69}{0.35} \\
        CIFAR-100 Coarse & 20 & 20,000 & \textbf{42.27 $\pm$ 0.17} &         42.04 $\pm$ 0.15  & \diff{-0.23}{0.31}\\
        CIFAR-100 Coarse & 20 & 10,000 &         38.96 $\pm$ 0.12  & \textbf{39.12 $\pm$ 0.28} & \diff{1.15}{0.38} \\
        CIFAR-100 Coarse & 20 &  5,000 &         33.52 $\pm$ 0.39  & \textbf{35.12 $\pm$ 0.25} & \diff{1.60}{0.50} \\
        CIFAR-100 Coarse & 20 &  1,000 &         22.21 $\pm$ 0.60  & \textbf{22.79 $\pm$ 0.24} & \diff{0.59}{0.36} \\
        CIFAR-100 Coarse & 20 &    500 &         18.54 $\pm$ 0.21  & \textbf{19.55 $\pm$ 0.56} & \diff{1.01}{0.74} \\
        CIFAR-100 Coarse & 20 &    100 &         11.28 $\pm$ 0.49  & \textbf{12.49 $\pm$ 0.40} & \diff{1.21}{0.11} \\
        \hhline{:===::===:}
        % converted to std error
        CIFAR-100 & 100 & 50,000 & 36.56 $\pm$ 0.35 & \textbf{40.93 $\pm$ 0.25} & \diff{4.38}{0.25} \\
        CIFAR-100 & 100 & 20,000 & 29.68 $\pm$ 0.18 & \textbf{32.82 $\pm$ 0.63} & \diff{3.14}{0.55} \\
        CIFAR-100 & 100 & 10,000 & 24.68 $\pm$ 0.79 & \textbf{27.66 $\pm$ 0.26} & \diff{2.99}{0.73} \\
        CIFAR-100 & 100 &  5,000 & 18.26 $\pm$ 0.36 & \textbf{22.50 $\pm$ 0.48} & \diff{4.24}{0.41} \\
        CIFAR-100 & 100 &  1,000 &  9.45 $\pm$ 0.27 & \textbf{11.01 $\pm$ 0.37} & \diff{1.56}{0.22} \\
        \hhline{:===::===:}
        % converted to std error
        Tiny-ImageNet & 200 & 100,000 &           18.95 $\pm$ 0.87 & \textbf{          25.43 $\pm$ 0.20} & \diff{6.48}{0.67} \\
        Tiny-ImageNet & 200 &  50,000 &           15.26 $\pm$ 0.25 & \textbf{          22.20 $\pm$ 0.42} & \diff{6.94}{0.18} \\
        Tiny-ImageNet & 200 &  20,000 &           12.14 $\pm$ 0.15 & \textbf{          15.65 $\pm$ 0.05} & \diff{3.51}{0.17} \\
        Tiny-ImageNet & 200 &  10,000 & \phantom{0}8.51 $\pm$ 0.06 & \textbf{          10.85 $\pm$ 0.29} & \diff{2.35}{0.35} \\
        Tiny-ImageNet & 200 &   5,000 & \phantom{0}6.34 $\pm$ 0.11 & \textbf{\phantom{0}7.94 $\pm$ 0.15} & \diff{1.60}{0.13} \\
	    \hhline{|---||---|}
	\end{tabularx}
	\vspace{-3ex}
\end{table*}

% \begin{table*}[t!]
%   \caption{Results on single label datasets.}
%   \label{tab:results-single-label}
%   \begin{center}
%   \begin{small}
%   \begin{sc}
%     \begin{tabular}{crrcc|r}
%     \toprule
%       \multirow{2}{*}{\textbf{Task}} & \multirow{ 2}{*}{\textbf{\#classes}} & \multirow{ 2}{*}{\textbf{\# samples}}& \multicolumn{3}{c}{\textbf{Accuracy}} \\ 
%       & & &  \textbf{baseline} & \textbf{curriculum} & \textbf{difference}\\
%       \hline
%       CIFAR-10  &  0.73  & $50,000$ & $71.08 \pm 0.50 $ & $\mathbf{71.81 \pm 0.16}$ & $0.73 \pm 0.57$ \\
%       CIFAR-10  &  $10$  & $20,000$ & $ 64.99 \pm 0.55 $ & $64.92 \pm 0.76$ & $ -0.07 \pm 0.92$ \\
%       CIFAR-10  &  $10$  & $10,000$ & $ 60.94 \pm 0.42 $ & $\mathbf{61.42 \pm 0.61}$ & $  0.48 \pm 0.43$ \\
%       CIFAR-10  &  $10$  &  $5,000$ & $ 55.89 \pm 0.83 $ & $\mathbf{56.84 \pm 0.93}$ & $	0.95 \pm 0.81	$\\
%       CIFAR-10  &  $10$  & $1,000$ & $42.52 \pm 1.44$ & $\mathbf{43.78 \pm 0.52}$ & $1.26 \pm 1.36$\\
%       CIFAR-10  &  $10$  &   $500$ & $37.754 \pm 1.26$ & $\mathbf{39.23 \pm 1.53}$ &  $1.47 \pm 0.83$ \\
%       CIFAR-10  &  $10$  &   $100$ & 24.13 & \textbf{28.85} & 4.72 \\
%       \hline
%       CIFAR-100 &  $100$ & $50,000$ & $36.56 \pm 0.79$ & $\mathbf{40.93 \pm 0.57}$ & $4.38 \pm 0.56$\\
%       CIFAR-100 &  $100$ & $20,000$ & $29.68 \pm 0.40$ & $\mathbf{32.82 \pm 1.4}$ & $3.14 \pm 1.23$\\
%       CIFAR-100 &  $100$ & $10,000$ & $24.68 \pm 1.78$ & $\mathbf{27.66 \pm 0.58}$ & $2.99 \pm 1.64$\\
%       CIFAR-100 &  $100$ &  $5,000$ & $18.26 \pm 0.81$ & $\mathbf{22.50 \pm 1.07}$ & $4.24 \pm 0.92$\\
%       CIFAR-100 &  $100$ &  $1,000$ & $ 9.45 \pm 0.60$ & $\mathbf{11.01 \pm 0.82}$ & $1.56 \pm 0.49$\\
%       \hline
%       SVHN     &  10  & 50,000 & \textbf{89.69} & 89.62 & -0.07\\
%       SVHN     &  10  & 20,000 & \textbf{86.64} & 84.88 & -1.76 \\
%       SVHN     &  10  & 10,000 & \textbf{83.52} & 83.12 & -0.4 \\
%       SVHN     &  10  &  5,000 & \textbf{81.31} & 80.18 & -1.13\\
%       SVHN     &  10  &  1,000 & 69.21 & \textbf{72.46} & 3.25 \\
%       SVHN     &  10  &    500 & 57.75 & \textbf{62.79} & 5.04 \\
%       SVHN     &  10  &    100 & 19.13 & \textbf{22.53} & 3.40 \\
%       \hline
%       Tiny-ImageNet & $200$ &  $100,000$ & $18.95 \pm 1.95$ & $\mathbf{25.43 \pm 0.45}$ & $6.48 \pm 1.49$ \\
%     \bottomrule
%     \end{tabular}
%     \end{sc}
%     \end{small}
%   \end{center}
% \end{table*}


==> tables/table-results-blobs.tex <==
\begin{table}[h!]
  \begin{center}
    \begin{tabular}{ccccc}
      \multirow{2}{*}{\textbf{Task}} & \multirow{ 2}{*}{\textbf{\#classes}} & \multirow{ 2}{*}{\textbf{\# samples}}& \multicolumn{2}{c}{\textbf{Accuracy}} \\ 
      & & &  \textbf{baseline} & \textbf{curriculum}\\
      \hline
      Blobs  &  7 & 100   & 30.7 & \textbf{34.3} \\
      Blobs  &  7 & 500   & \textbf{39.0} & 38.0 \\
      Blobs  &  7 & 1000  & 43.5 & \textbf{46.5} \\

    \end{tabular}
  \end{center}
  \caption{Results on Gaussian blobs datasets.}
   \label{tab:results-blobs}
\end{table}


==> tables/table-results-shapes.tex <==
\begin{table}[h!]
  \begin{center}
    \begin{tabular}{cccc}
      \multirow{2}{*}{\textbf{Task}} & \textbf{\#samples}& \multicolumn{2}{c}{\textbf{Accuracy}} \\ 
      &  \textbf{per class} &  \textbf{baseline} & \textbf{curriculum}\\
     \hline
    Polygons & 100   & 14.53 $\pm$ 1.06 & \textbf{15.63} $\pm$ 2.93\\
    Polygons & 200	  & 17.34 $\pm$ 3.05 & \textbf{18.91} $\pm$ 4.42\\
    Polygons & 300   & 21.98 $\pm$ 1.90 & \textbf{24.22} $\pm$ 4.98\\
    Polygons & 500	  & 29.67 $\pm$ 2.84 & \textbf{38.03} $\pm$ 3.92\\
    Polygons & 700	  & 37.48 $\pm$ 1.21 & \textbf{47.32} $\pm$ 1.59\\
    Polygons & 1000  & 48.87 $\pm$ 4.73 & \textbf{60.92} $\pm$ 2.34\\
    Polygons & 5000  & \textbf{96.66} $\pm$ 0.89 & 96.45 $\pm$ 0.13\\
    \end{tabular}
  \end{center}
  \caption{Results on shapes datasets.}
   \label{tab:results-shapes}
\end{table}
